Characteristic Timescales of the Local Moment Dynamics in Hund's-metals

We study the characteristic time scales of the fluctuating local moments in Hund's metal systems for different degrees of correlation. By analyzing the dynamical spin susceptibility in the real-time domain via the fluctuation-dissipation theorem, we determine the time scales controlling oscillation and damping of on-site fluctuations - a crucial factor for the detection of local moments with different experimental probes. We apply this procedure to realistic many-body calculations of different families of iron-pnictides and chalcogenides, explaining the material-specific trend in the discrepancies reported between experimental and theoretical estimates of the magnetic moments.

==> tab/tab_fit_timescales.tex <==
\begin{table*}[h!]
\centering
\ra{1.3}
\begin{tabular}{@{}lcccccc@{}}\toprule
 	 				&	&LaFeAsO	&BaFe$_2$As$_2$	&LiFeAs		&KFe$_2$As$_2$	&FeTe	  \\
\midrule
$\omega_{\text{max peak}_1}$	& [$\mathrm{eV}$]&0.2488	&0.1574		&0.0751		&0.0562		&0.0245	\\
$t_{\text{max peak}_1}$ & [$\mathrm{fs}$]		&2.65		&4.18		&8.76		&11.70		&26.91		\\
$t_{\omega0_1}$	       & [$\mathrm{fs}$]		&1.92		&(2.61)		&1.45		&0.54		&18.97		\\
$t_{\gamma_1}$	       & [$\mathrm{fs}$]		&(\tb{2.33})&\tb{2.48}	&(2.68)		&(1.84)		&(\tb{23.94})	\\
$t_{\omega_1}$	       & [$\mathrm{fs}$]		&3.41		&7.96		&\tb{1.72}	&\tb{0.57}	&31.09		\\
$\omega_{\text{max peak}_2}$ & [$\mathrm{eV}$]	&	-		&	-		&	-		&-			&0.3228		\\
$t_{\text{max peak}_2}$ & [$\mathrm{fs}$]		&	-		&	-		&	-		&-			&2.04		\\
$t_{\omega0_2}$		& [$\mathrm{fs}$]			&	-		&	-		&	-		&-			&1.84		\\
$t_{\gamma_2}$		& [$\mathrm{fs}$]			&	-		&	-		&	-		&-			&(5.92)		\\
$t_{\omega_2}$		& [$\mathrm{fs}$]			&	-		&	-		&	-		&-			&\tb{1.93}	\\
\bottomrule
\end{tabular}
\caption{Peak-locations of the MaxEnt data and timescales of the fits for all considered materials with $full$ $ U$-interaction in the $d-$model. }
\label{tab:timescales}
\end{table*}
	

